ALMA [CII] 158um imaging of an HI-Selected Major Merger at z~4

We present high spatial-resolution (~2kpc) Atacama Large Millimeter/submillimeter Array (ALMA) observations of [CII] 158um and dust-continuum emission from a galaxy at z=3.7978 selected by its strong HI absorption (a damped Lya absorber, DLA) against a background QSO. Our ALMA images reveal a pair of star-forming galaxies separated by ~6kpc (projected) undergoing a major merger. Between these galaxies is a third emission component with highly elevated (2x) [CII] 158um emission relative to the dust continuum, which is likely to arise from stripped gas associated with the merger. This merger of two otherwise-normal galaxies is not accompanied by enhanced star-formation, contrary to mergers detected in most luminosity-selected samples. The DLA associated with the merger exhibits extreme kinematics, with a velocity width for the low-ionization metal lines of Dv90~470km/s that spans the velocity spread revealed in the [CII] 158um emission. We propose that DLAs with high Dv90 values are a signpost of major mergers in normal galaxies at high redshifts, and use the distribution of the velocity widths of metal lines in high-z DLAs to provide a rough estimate the fraction of z>3 galaxies that are undergoing a major merger.

==> table1.tex <==
\begin{deluxetable*}{cccccc}
\tablewidth{0pc}
\tablecaption{MEASUREMENTS\label{tab:values}}
\tabletypesize{\footnotesize}
\tablehead{\colhead{Quantity}  & \colhead{Unit} 
& \colhead{Component-A$^a$} 
& \colhead{Component-B} 
& \colhead{Component-C} 
& \colhead{Total} 
\\ 
 } 
\startdata 
$\int S_{\rm [CII]} \, dv$ & Jy km s$^{-1}$& $0.51 \pm 0.007$ & $0.51 \pm 0.006$ & $0.34 \pm  0.005$ & $1.36 \pm 0.010$ \\ 
\lcplus & $10^8 \, L_\odot$& $2.5 \pm 0.0$ & $2.5 \pm 0.0$ & $1.7 \pm 0.0$ & $6.6 \pm 0.1$\\ 
$f_{\rm IR}$ & mJy& $0.133 \pm 0.003$ & $0.097 \pm 0.003$ & $0.039 \pm 0.002$ & $0.269 \pm 0.005$ \\ 
$L_{\rm IR}^b$ & $10^{10} L_\odot$& $10.0 \pm 0.2$ & $7.2 \pm 0.2$ & $2.9 \pm 0.2$ & $20.1 \pm 0.4$ \\ 
SFR & M$_\odot$ yr$^{-1}$& $10.8 \pm 0.3$ & $7.8 \pm 0.2$ & $3.1 \pm 0.2$ & $21.8 \pm 0.4$\\ 
$v$ & km/s& 44.4 & 1.7 & 7.7 & 19.3 \\ 
\hline 
\enddata 
\tablenotetext{a}{Components A, B and C are defined relative to \origpos\ in Section~\ref{sec:obs}.}
\tablenotetext{b}{The total IR luminosity for $\lambda = 8-1000 \mu$m, estimated from the continuum flux density, assuming a modified blackbody spectrum with $T=35$\,K and $$\beta = 1.6$.}
\end{deluxetable*} 

